Extensionless Adaptive Transmitter and Receiver Windowing of Beyond 5G Frames

Newer cellular communication generations are planned to allow asynchronous transmission of multiple numerologies (waveforms with different parameters) in adjacent bands, creating unavoidable adjacent channel interference. Most prior work on windowing assume additional extensions reserved for windowing, which does not comply with standards. Whether windowing should be applied at the transmitter or the receiver was not questioned. In this work, we propose two independent algorithms that are implemented at the transmitter and receiver, respectively. These algorithms estimate the transmitter and receiver windowing duration of each resource element (RE) with an aim to improve fair proportional network throughput. While doing so, we solely utilize the available extension that was defined in the standard and present standard-compliant algorithms that also do not require any modifications on the counterparts or control signaling. Furthermore, computationally efficient techniques to apply per-RE transmitter and receiver windowing to signals synthesized and analyzed using conventional cyclic prefix orthogonal frequency division multiplexing are derived and their computational complexities are analyzed. The spectrotemporal relations between optimum window durations at either side, as well as functions of the excess signal to noise ratios, the subcarrier spacings and the throughput gains provided over previous similar techniques are numerically verified.

==> FINAL SUBMISSION PACK/acros.tex <==
% Extend acronym package with first letter caps
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother
% Acronyms
\acrodef{ofdm}[OFDM]{orthogonal frequency division multiplexing}
\acrodef{fofdm}[F-OFDM]{filtered-\aclu{ofdm}}
\acrodef{fbmc}[FBMC]{filter bank multicarrier}
\acrodef{fmt}[FMT]{filtered multitone}
\acrodef{ufmc}[UFMC]{universal filtered multicarrier}
\acrodef{gfdm}[GFDM]{generalized frequency division multiplexing}
\acrodef{zf}[ZF]{zero forcing}
\acrodef{mimo}[MIMO]{multiple-input-multiple-output}
\acrodef{siso}[SISO]{single-input single-output}
\acrodef{np}[NP]{nondeterministic polynomial}
\acrodef{sc}[SC]{single carrier}
\acrodef{sc-fde}[SC-FDE]{\aclu{sc}-\aclu{fde}}
\acrodef{evm}[EVM]{error vector magnitude}
\acrodef{dft}[DFT]{discrete Fourier transformation}
\acrodef{ifft}[IFFT]{inverse fast Fourier transformation}
\acrodef{cp}[CP]{cyclic prefix}
\acrodef{papr}[PAPR]{peak-to-average power ratio}
\acrodef{qam}[QAM]{quadrature amplitude modulation}
\acrodef{ask}[ASK]{amplitude shift keying}
\acrodef{psk}[PSK]{phase shift keying}
\acrodef{apsk}[APSK]{amplitude phase shift keying}
\acrodef{fsk}[FSK]{frequency shift keying}
\acrodef{gmsk}[GMSK]{gaussian minimum shift keying}
\acrodef{im}[IM]{index modulation}
\acrodef{fft}[FFT]{fast Fourier transformation}
\acrodef{ici}[ICI]{inter-carrier interference}
\acrodef{isi}[ISI]{intersymbol interference}
\acrodef{ini}[INI]{inter-numerology interference}
\acrodef{pdf}[PDF]{probability density function}
\acrodef{cr}[CR]{cognitive radio}
\acrodef{wola}[WOLA]{weighted overlap-add}
\acrodef{qos}[QoS]{Quality of Service}
\acrodef{csi}[CSI]{channel state information}
\acrodef{ber}[BER]{bit-error rate}
\acrodef{rf}[RF]{radio frequency}
\acrodef{rrc}[RRC]{root-raised cosine}
\acrodef{as}[AS]{alignment signal}
\acrodef{snr}[SNR]{signal-to-noise ratio}
\acrodef{dfe}[DFE]{decision-feedback equalizer}
\acrodef{fde}[FDE]{frequency domain equalization}
\acrodef{oob}[OOB]{out-of-band}
\acrodef{aci}[ACI]{adjacent channel interference}
\acrodef{naci}[NACI]{noise-plus-\aclu{aci}}
\acrodef{phy}[PHY]{physical layer}
\acrodef{mse}[MSE]{mean-square error}
\acrodef{pa}[PA]{power amplifier}
\acrodef{rb}[RB]{resource block}
\acrodef{ran}[RAN]{radio-access network}
\acrodef{rat}[RAT]{radio access technology}
\acrodefplural{rat}[RATs]{radio access technologies}
\acrodef{mmwave}[mmWave]{millimeter wave}
\acrodef{3gpp}[3GPP]{Third Generation Partnership Project}
\acrodef{sc}[SC]{single carrier}
\acrodef{uw}[UW]{unique word}
\acrodef{zt}[ZT]{zero tail}
\acrodef{gi}[GI]{guard interval}
\acrodef{sinr}[SINR]{signal to interference plus noise ratio}
\acrodef{dpss}[DPSS]{discrete prolate spheroidal sequences}
\acrodef{bler}[BLER]{block error rate}
\acrodef{fdd}[FDD]{frequency domain duplexing}
\acrodef{tdd}[TDD]{time domain duplexing}
\acrodef{ul}[UL]{uplink}
\acrodef{dl}[DL]{downlink}
\acrodef{bs}[BS]{base station}
\acrodef{af}[AF]{ambiguity function}
\acrodef{ms}[MS]{mobile station}
\acrodef{iot}[IoT]{Internet of Things}
\acrodef{pdp}[PDP]{power delay profile}
\acrodef{ftn}[FTN]{Faster-than-Nyquist}
\acrodef{svd}[SVD]{singular-value decomposition}
\acrodef{uw-ofdm}[UW-OFDM]{\aclu{uw}-\aclu{ofdm}}
\acrodef{w-ofdm}[W-OFDM]{windowed-\aclu{ofdm}}
\acrodef{rw-ofdm}[RW-OFDM]{receiver \aclu{w-ofdm}}
\acrodef{cp-ofdm}[CP-OFDM]{\aclu{cp}-\aclu{ofdm}}
\acrodef{dft-s-ofdm}[DFT-s-OFDM]{\aclu{dft}-spread-\aclu{ofdm}}
\acrodef{lte}[LTE]{Long Term Evolution}
\acrodef{lte-a}[LTE-A]{\aclu{lte}-Advanced}
\acrodef{gsm}[GSM]{Global System for Mobile Communications}
\acrodef{ma}[MA]{multiple accessing}
\acrodef{oma}[OMA]{orthogonal multiple accessing}
\acrodef{noma}[NOMA]{non-orthogonal multiple accessing}
\acrodef{cdnoma}[CD-NOMA]{code domain \aclu{noma}}
\acrodef{pdnoma}[PD-NOMA]{power domain \aclu{noma}}
\acrodef{fdma}[FDMA]{frequency division multiple accessing}
\acrodef{ofdma}[OFDMA]{orthogonal frequency division multiple accessing}
\acrodef{sc-fdma}[SC-FDMA]{single carrier-frequency division multiple accessing}
\acrodef{cdma}[CDMA]{code division multiple accessing}
\acrodef{tdma}[TDMA]{time division multiple accessing}
\acrodef{embb}[eMBB]{enhanced-mobile broadband}
\acrodef{mmtc}[mMTC]{massive machine type communications}
\acrodef{urllc}[uRLLC]{ultra reliable and low latency communications}
\acrodef{dvb}[DVB]{digital video broadcasting}
\acrodef{comp}[CoMP]{Coordinated Multi Point}
\acrodef{jt-comp}[JT-CoMP]{Joint Transmission-\aclu{comp}}
\acrodef{sic}[SIC]{successive interference cancellation}
\acrodef{osic}[OSIC]{ordered successive interference cancellation}
\acrodef{ml}[ML]{maximum likelihood}
\acrodef{sl}[SL]{sidelink}
\acrodef{qpsk}[QPSK]{quadrature phase shift keying}
\acrodef{mpa}[MPA]{message passing algorithm}
\acrodef{amc}[AMC]{adaptive modulation and coding}
\acrodef{umts}[UMTS]{Universal Mobile Telecommunications Service}
\acrodef{e-utra}[E-UTRA]{Evolved \aclu{umts} Terrestrial Radio Access}
\acrodef{ue}[UE]{user equipment}
\acrodef{harq}[HARQ]{hybrid automatic repeat request}
\acrodef{nr}[NR]{new radio}
\acrodef{hetnet}[HetNet]{heterogeneous network}
\acrodef{pot}[POT]{partially overlapping tones}
\acrodef{rms}[RMS]{root mean square}
\acrodef{must}[MUST]{multiuser superposition transmission}
\acrodef{csma}[CSMA]{carrier sense \aclu{ma}}
\acrodef{sdma}[SDMA]{space division \aclu{ma}}
\acrodef{mno}[MNO]{mobile network operator}
\acrodef{d2d}[D2D]{device-to-device}
\acrodef{v2v}[V2V]{vehicle-to-vehicle}
\acrodef{v2x}[V2X]{vehicle-to-infrastructure}
\acrodef{med}[MED]{maximum excess delay}
\acrodef{awgn}[AWGN]{additive white Gaussian noise}
\acrodef{cfr}[CFR]{channel frequency response}
\acrodef{cir}[CIR]{channel impulse response}
\acrodef{sir}[SIR]{signal-to-interference ratio}
\acrodef{lut}[LUT]{lookup table}
\acrodef{ssw}[SSW]{subcarrier specific window}
\acrodef{cqi}[CQI]{channel quality indicator}
\acrodef{bpsk}[BPSK]{binary phase shift keying}
\acrodef{mcs}[MCS]{modulation and coding scheme}
\acrodef{dac}[DAC]{digital-to-analog converter}
\acrodef{ncofdm}[NC-OFDM]{$N$-Continuous \aclu{ofdm}}
\acrodef{adc}[ADC]{analog-to-digital converter}
\acrodef{e2e}[E2E]{end-to-end}
\acrodef{kpi}[KPI]{key performance indicator}
\acrodef{p1db}[P1dB]{1 dB compression point}
\acrodef{sqnr}[SQNR]{signal-to-quantization-noise ratio}
\acrodef{cmos}[CMOS]{complementary metal–oxide–semiconductor}
\acrodef{cs}[CS]{cyclic suffix}
\acrodef{pn}[PN]{phase noise}
\acrodef{xo}[XO]{crystal oscillator}
\acrodef{dc}[DC]{direct current}
\acrodef{ac}[AC]{alternating current}
\acrodef{ss}[SS]{spread spectrum}
\acrodef{dsss}[DSSS]{direct sequence \aclu{ss}}
\acrodef{fhss}[FHSS]{frequency hopping \aclu{ss}}
\acrodef{gps}[GPS]{global positioning system}
\acrodef{ap}[AP]{access point}
\acrodef{rts}[RTS]{request to send}
\acrodef{cts}[CTS]{clear to send}
\acrodef{macaw}[MACAW]{multiple access collision avoidance for wireless}
\acrodef{sifs}[SIFS]{short interframe space}
\acrodef{ssid}[SSID]{service set identifier}
\acrodef{mu}[MU]{multi-user}
\acrodef{sta}[STA]{station}
\acrodef{wcsp}[WCSP]{Wireless Communications and Signal Processing}
\acrodef{metu}[METU]{Middle East Technical University}
\acrodef{njit}[NJIT]{New Jersey Institute of Technology}
\acrodef{usf}[USF]{University of South Florida}
\acrodef{nnrp}[NNRP]{network normalized received power}
\acrodef{mrc}[MRC]{maximum ratio combining}
\acrodef{uci}[UCI]{uplink channel information}
\acrodef{map}[MAP]{maximum a posteriori}
\acrodef{ls}[LS]{least squares}
\acrodef{mai}[MAI]{multiple access interference}
\acrodef{gmm}[GMM]{Gaussian mixture model}
\acrodef{pca}[PCA]{principal component analysis}
\acrodef{prb}[PRB]{physical resource block}
\acrodef{tti}[TTI]{transmission time interval}
\acrodef{tdl}[TDL]{tapped delay line}
\acrodef{llr}[LLR]{log-likelihood ratio}
\acrodef{re}[RE]{resource element}
\acrodef{gnb}[gNB]{next generation NodeB}
\acrodef{pusch}[PUSCH]{physical uplink shared channel}
\acrodef{ldpc}[LDPC]{low density parity check}
\acrodef{psd}[PSD]{power spectral density}
\acrodef{dmrs}[DMRS]{demodulation reference signal}
\acrodef{bch}[BCH]{Bose–Chaudhuri–Hocquenghem} % \cite{Bose1960} \cite{Hocquenghem1959}
\acrodef{sg}[SG]{subcarrier group}
\acrodef{bwp}[BWP]{bandwidth part}
\acrodef{tpc}[TPC]{Turbo product code}
\acrodef{pam}[PAM]{pulse amplitude modualation}
\acrodef{lmmse}[LMMSE]{linear minimum mean square error}


==> acros.tex <==
% Extend acronym package with first letter caps
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother
% Acronyms
\acrodef{ofdm}[OFDM]{orthogonal frequency division multiplexing}
\acrodef{fofdm}[F-OFDM]{filtered-\aclu{ofdm}}
\acrodef{fbmc}[FBMC]{filter bank multicarrier}
\acrodef{fmt}[FMT]{filtered multitone}
\acrodef{ufmc}[UFMC]{universal filtered multicarrier}
\acrodef{gfdm}[GFDM]{generalized frequency division multiplexing}
\acrodef{zf}[ZF]{zero forcing}
\acrodef{mimo}[MIMO]{multiple-input-multiple-output}
\acrodef{siso}[SISO]{single-input single-output}
\acrodef{np}[NP]{nondeterministic polynomial}
\acrodef{sc}[SC]{single carrier}
\acrodef{sc-fde}[SC-FDE]{\aclu{sc}-\aclu{fde}}
\acrodef{evm}[EVM]{error vector magnitude}
\acrodef{dft}[DFT]{discrete Fourier transformation}
\acrodef{ifft}[IFFT]{inverse fast Fourier transformation}
\acrodef{cp}[CP]{cyclic prefix}
\acrodef{papr}[PAPR]{peak-to-average power ratio}
\acrodef{qam}[QAM]{quadrature amplitude modulation}
\acrodef{ask}[ASK]{amplitude shift keying}
\acrodef{psk}[PSK]{phase shift keying}
\acrodef{apsk}[APSK]{amplitude phase shift keying}
\acrodef{fsk}[FSK]{frequency shift keying}
\acrodef{gmsk}[GMSK]{gaussian minimum shift keying}
\acrodef{im}[IM]{index modulation}
\acrodef{fft}[FFT]{fast Fourier transformation}
\acrodef{ici}[ICI]{inter-carrier interference}
\acrodef{isi}[ISI]{intersymbol interference}
\acrodef{ini}[INI]{inter-numerology interference}
\acrodef{pdf}[PDF]{probability density function}
\acrodef{cr}[CR]{cognitive radio}
\acrodef{wola}[WOLA]{weighted overlap-add}
\acrodef{qos}[QoS]{Quality of Service}
\acrodef{csi}[CSI]{channel state information}
\acrodef{ber}[BER]{bit-error rate}
\acrodef{rf}[RF]{radio frequency}
\acrodef{rrc}[RRC]{root-raised cosine}
\acrodef{as}[AS]{alignment signal}
\acrodef{snr}[SNR]{signal-to-noise ratio}
\acrodef{dfe}[DFE]{decision-feedback equalizer}
\acrodef{fde}[FDE]{frequency domain equalization}
\acrodef{oob}[OOB]{out-of-band}
\acrodef{aci}[ACI]{adjacent channel interference}
\acrodef{naci}[NACI]{noise-plus-\aclu{aci}}
\acrodef{phy}[PHY]{physical layer}
\acrodef{mse}[MSE]{mean-square error}
\acrodef{pa}[PA]{power amplifier}
\acrodef{rb}[RB]{resource block}
\acrodef{ran}[RAN]{radio-access network}
\acrodef{rat}[RAT]{radio access technology}
\acrodefplural{rat}[RATs]{radio access technologies}
\acrodef{mmwave}[mmWave]{millimeter wave}
\acrodef{3gpp}[3GPP]{Third Generation Partnership Project}
\acrodef{sc}[SC]{single carrier}
\acrodef{uw}[UW]{unique word}
\acrodef{zt}[ZT]{zero tail}
\acrodef{gi}[GI]{guard interval}
\acrodef{sinr}[SINR]{signal to interference plus noise ratio}
\acrodef{dpss}[DPSS]{discrete prolate spheroidal sequences}
\acrodef{bler}[BLER]{block error rate}
\acrodef{fdd}[FDD]{frequency domain duplexing}
\acrodef{tdd}[TDD]{time domain duplexing}
\acrodef{ul}[UL]{uplink}
\acrodef{dl}[DL]{downlink}
\acrodef{bs}[BS]{base station}
\acrodef{af}[AF]{ambiguity function}
\acrodef{ms}[MS]{mobile station}
\acrodef{iot}[IoT]{Internet of Things}
\acrodef{pdp}[PDP]{power delay profile}
\acrodef{ftn}[FTN]{Faster-than-Nyquist}
\acrodef{svd}[SVD]{singular-value decomposition}
\acrodef{uw-ofdm}[UW-OFDM]{\aclu{uw}-\aclu{ofdm}}
\acrodef{w-ofdm}[W-OFDM]{windowed-\aclu{ofdm}}
\acrodef{rw-ofdm}[RW-OFDM]{receiver \aclu{w-ofdm}}
\acrodef{cp-ofdm}[CP-OFDM]{\aclu{cp}-\aclu{ofdm}}
\acrodef{dft-s-ofdm}[DFT-s-OFDM]{\aclu{dft}-spread-\aclu{ofdm}}
\acrodef{lte}[LTE]{Long Term Evolution}
\acrodef{lte-a}[LTE-A]{\aclu{lte}-Advanced}
\acrodef{gsm}[GSM]{Global System for Mobile Communications}
\acrodef{ma}[MA]{multiple accessing}
\acrodef{oma}[OMA]{orthogonal multiple accessing}
\acrodef{noma}[NOMA]{non-orthogonal multiple accessing}
\acrodef{cdnoma}[CD-NOMA]{code domain \aclu{noma}}
\acrodef{pdnoma}[PD-NOMA]{power domain \aclu{noma}}
\acrodef{fdma}[FDMA]{frequency division multiple accessing}
\acrodef{ofdma}[OFDMA]{orthogonal frequency division multiple accessing}
\acrodef{sc-fdma}[SC-FDMA]{single carrier-frequency division multiple accessing}
\acrodef{cdma}[CDMA]{code division multiple accessing}
\acrodef{tdma}[TDMA]{time division multiple accessing}
\acrodef{embb}[eMBB]{enhanced-mobile broadband}
\acrodef{mmtc}[mMTC]{massive machine type communications}
\acrodef{urllc}[uRLLC]{ultra reliable and low latency communications}
\acrodef{dvb}[DVB]{digital video broadcasting}
\acrodef{comp}[CoMP]{Coordinated Multi Point}
\acrodef{jt-comp}[JT-CoMP]{Joint Transmission-\aclu{comp}}
\acrodef{sic}[SIC]{successive interference cancellation}
\acrodef{osic}[OSIC]{ordered successive interference cancellation}
\acrodef{ml}[ML]{maximum likelihood}
\acrodef{sl}[SL]{sidelink}
\acrodef{qpsk}[QPSK]{quadrature phase shift keying}
\acrodef{mpa}[MPA]{message passing algorithm}
\acrodef{amc}[AMC]{adaptive modulation and coding}
\acrodef{umts}[UMTS]{Universal Mobile Telecommunications Service}
\acrodef{e-utra}[E-UTRA]{Evolved \aclu{umts} Terrestrial Radio Access}
\acrodef{ue}[UE]{user equipment}
\acrodef{harq}[HARQ]{hybrid automatic repeat request}
\acrodef{nr}[NR]{new radio}
\acrodef{hetnet}[HetNet]{heterogeneous network}
\acrodef{pot}[POT]{partially overlapping tones}
\acrodef{rms}[RMS]{root mean square}
\acrodef{must}[MUST]{multiuser superposition transmission}
\acrodef{csma}[CSMA]{carrier sense \aclu{ma}}
\acrodef{sdma}[SDMA]{space division \aclu{ma}}
\acrodef{mno}[MNO]{mobile network operator}
\acrodef{d2d}[D2D]{device-to-device}
\acrodef{v2v}[V2V]{vehicle-to-vehicle}
\acrodef{v2x}[V2X]{vehicle-to-infrastructure}
\acrodef{med}[MED]{maximum excess delay}
\acrodef{awgn}[AWGN]{additive white Gaussian noise}
\acrodef{cfr}[CFR]{channel frequency response}
\acrodef{cir}[CIR]{channel impulse response}
\acrodef{sir}[SIR]{signal-to-interference ratio}
\acrodef{lut}[LUT]{lookup table}
\acrodef{ssw}[SSW]{subcarrier specific window}
\acrodef{cqi}[CQI]{channel quality indicator}
\acrodef{bpsk}[BPSK]{binary phase shift keying}
\acrodef{mcs}[MCS]{modulation and coding scheme}
\acrodef{dac}[DAC]{digital-to-analog converter}
\acrodef{ncofdm}[NC-OFDM]{$N$-Continuous \aclu{ofdm}}
\acrodef{adc}[ADC]{analog-to-digital converter}
\acrodef{e2e}[E2E]{end-to-end}
\acrodef{kpi}[KPI]{key performance indicator}
\acrodef{p1db}[P1dB]{1 dB compression point}
\acrodef{sqnr}[SQNR]{signal-to-quantization-noise ratio}
\acrodef{cmos}[CMOS]{complementary metal–oxide–semiconductor}
\acrodef{cs}[CS]{cyclic suffix}
\acrodef{pn}[PN]{phase noise}
\acrodef{xo}[XO]{crystal oscillator}
\acrodef{dc}[DC]{direct current}
\acrodef{ac}[AC]{alternating current}
\acrodef{ss}[SS]{spread spectrum}
\acrodef{dsss}[DSSS]{direct sequence \aclu{ss}}
\acrodef{fhss}[FHSS]{frequency hopping \aclu{ss}}
\acrodef{gps}[GPS]{global positioning system}
\acrodef{ap}[AP]{access point}
\acrodef{rts}[RTS]{request to send}
\acrodef{cts}[CTS]{clear to send}
\acrodef{macaw}[MACAW]{multiple access collision avoidance for wireless}
\acrodef{sifs}[SIFS]{short interframe space}
\acrodef{ssid}[SSID]{service set identifier}
\acrodef{mu}[MU]{multi-user}
\acrodef{sta}[STA]{station}
\acrodef{wcsp}[WCSP]{Wireless Communications and Signal Processing}
\acrodef{metu}[METU]{Middle East Technical University}
\acrodef{njit}[NJIT]{New Jersey Institute of Technology}
\acrodef{usf}[USF]{University of South Florida}
\acrodef{nnrp}[NNRP]{network normalized received power}
\acrodef{mrc}[MRC]{maximum ratio combining}
\acrodef{uci}[UCI]{uplink channel information}
\acrodef{map}[MAP]{maximum a posteriori}
\acrodef{ls}[LS]{least squares}
\acrodef{mai}[MAI]{multiple access interference}
\acrodef{gmm}[GMM]{Gaussian mixture model}
\acrodef{pca}[PCA]{principal component analysis}
\acrodef{prb}[PRB]{physical resource block}
\acrodef{tti}[TTI]{transmission time interval}
\acrodef{tdl}[TDL]{tapped delay line}
\acrodef{llr}[LLR]{log-likelihood ratio}
\acrodef{re}[RE]{resource element}
\acrodef{gnb}[gNB]{next generation NodeB}
\acrodef{pusch}[PUSCH]{physical uplink shared channel}
\acrodef{ldpc}[LDPC]{low density parity check}
\acrodef{psd}[PSD]{power spectral density}
\acrodef{dmrs}[DMRS]{demodulation reference signal}
\acrodef{bch}[BCH]{Bose–Chaudhuri–Hocquenghem} % \cite{Bose1960} \cite{Hocquenghem1959}
\acrodef{sg}[SG]{subcarrier group}
\acrodef{bwp}[BWP]{bandwidth part}
\acrodef{tpc}[TPC]{Turbo product code}
\acrodef{pam}[PAM]{pulse amplitude modualation}
\acrodef{lmmse}[LMMSE]{linear minimum mean square error}

